CaPo: Cooperative Plan Optimization for Efficient Embodied Multi-Agent Cooperation

In this work, we address the cooperation problem among large language model (LLM) based embodied agents, where agents must cooperate to achieve a common goal. Previous methods often execute actions extemporaneously and incoherently, without long-term strategic and cooperative planning, leading to redundant steps, failures, and even serious repercussions in complex tasks like search-and-rescue missions where discussion and cooperative plan are crucial. To solve this issue, we propose Cooperative Plan Optimization (CaPo) to enhance the cooperation efficiency of LLM-based embodied agents. Inspired by human cooperation schemes, CaPo improves cooperation efficiency with two phases: 1) meta-plan generation, and 2) progress-adaptive meta-plan and execution. In the first phase, all agents analyze the task, discuss, and cooperatively create a meta-plan that decomposes the task into subtasks with detailed steps, ensuring a long-term strategic and coherent plan for efficient coordination. In the second phase, agents execute tasks according to the meta-plan and dynamically adjust it based on their latest progress (e.g., discovering a target object) through multi-turn discussions. This progress-based adaptation eliminates redundant actions, improving the overall cooperation efficiency of agents. Experimental results on the ThreeDworld Multi-Agent Transport and Communicative Watch-And-Help tasks demonstrate that CaPo achieves much higher task completion rate and efficiency compared with state-of-the-arts.The code is released at https://github.com/jliu4ai/CaPo.

==> table/num_agents.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\setlength{\tabcolsep}{0.7mm}
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcc}
\toprule
& \textbf{Symbolic Obs ($\downarrow$)} & \textbf{Visual Obs ($\downarrow$)} \\ \hline
\textbf{CaPo}   &  93           &  106          \\
\textbf{CaPo$\times$2} &  51            &   83   \\
\textbf{CaPo$\times$3} &   46           &  \textbf{72}          \\ 
\textbf{CaPo$\times$4} &  \textbf{45}            &  74       \\ 
\bottomrule
\end{tabular}}
\vspace{-2mm}
\caption{\textbf{Benefits of increasing agent numbers in our CaPo on  the C-WAH task}. Average steps required to complete task are reported.}
\label{table:agent_num}
\end{wraptable}
